VOCABTRIM: Vocabulary Pruning for Efficient Speculative Decoding in LLMs

In this paper, we introduce a simple training-free technique to improve the performance of drafter-based speculative decoding (SpD) methods that incorporates language modeling head (LM head) during drafting process. A drafter-based speculative decoding leverages one or more smaller language models, a.k.a. drafters or draft models, to sample a draft sequence or tree consisting of multiple tokens, followed by verification by a base LLM, a target model, accepting a subset as its valid generation. As it is usually considered that the speculative decoding requires one-to-one mapping between vocabularies of the target model and the draft model, it has been natural to share the vocabulary between them, or even share the LM head as in EAGLE or Medusa. We first identify that this draft token sampling scheme inherently contains an unnecessary inference overhead in drafting, especially for some target LLMs with very large vocabularies. Then, we propose a simple technique, VocabTrim, to mitigate the drafting overhead to improve the generation speed in memory-bound environment. VocabTrim reconstructs the drafter LM head to contain only a limited set of tokens, selected by the most frequently sampled from the vocabulary of the target model. While limiting the vocabulary in drafting slightly degrades the acceptance rate, it significantly reduces the drafting latency in memory-bound process which is often the case on edge devices, resulting in higher memory-bound speed up (MBSU). We show that our method can boost the memory-bound speed-up for Llama-3 models on Spec-Bench, specifically by 16% for Llama-3.2-3B-Instruct.

==> contents/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}
% \begin{itemize}
%     \item SPD and details: memory bound, etc.
%     \item draft model is small and has limited representation, cannot cover entire vocab space, especially for recent SOTA models with high vocab dimension
%     \item draft model vocab can be efficiently reduced based on down-stream task: function-calling task such as XLAM only uses $xx$ number of tokens while open-ended text generation task such as Dolly has the following token distribution based on LLama3 generation. Analogous to how LORA adapters are an efficient way of improving LLM performance for a particular downstream task, we prpose a training-free method for increasing throughput of LLM based on the frequency of token occurence. 
% \end{itemize}
Since the inception of Speculative decoding (SpD) \cite{leviathan2023fast}, there have been several methods that have improved its performance in memory-bound systems. One common method is to draft multiple trajectories of tokens instead of a single sequence to increase the likelihood of acceptance \cite{RSD}, \cite{SpecInfer} . Another approach is to replace the independent drafter model with a smaller number of trainable parameters, such as the approaches taken by Medusa \cite{} SSD \cite{}. These method are not mututally exclusive, as we see the current SOTA \cite{EAGLE3} combining them in an effective manner. The majority of speculative decoding systems propose similar structures, using a smaller drafter model to propose candidate tokens and larger target model used for verification. 
Interestingly, all these methods use a drafter model  for generating speculative tokens operating in the same vocabulary space as the larger target model, even though the drafter model is much smaller than base model, \SA{I think we need references other than TVD++ here - what size draft do the other papers use?} \cite{TVD++} used drafter model of size $115$M for $7$B target model, \SA{this is the main point - we should reword it for clarity and impact.} and draft has limited representation power and has been observed to predict easy words (articles, prepositions, etc.) or completing half generated words (generating "table", when target model generation "vege") \cite{SPD-MLLM}. 

The draft model is usually trained separately from the target model following the usual pipeline of pretraining and supervised finetuning, often using a distillation dataset generated from the target model \cite{TVD++}. Methods improving vanilla SpD also involve cumbersome training with high compute resources \cite{Eagle, Mixutre of attention, Medusa}. In this paper, we emphasize a training-free method which may be integrated seamlessly into any existing SpD systems. 

Recently, large language models have seen a shift from smaller vocabulary sizes, from $32$K in Llama2 model family \cite{}), to a four-fold increase in Llama3, QWen2.5 model families to $128$K. A larger vocabulary can help provide the target LLM with multi-lingual capabilities and additionally improve representation power \cite{scaling law with vocab}. However, from the perspective of drafter model whose sole purpose is to speculate tokens aligned with target model distribution, there has been no study on the impact of vocabulary size of drafter models during speculative decoding. The drafter model is considerably smaller than base model, \cite{TVD++}, therefore, has much lower representation power (high perplexity). In this paper, we ask the question, \textit{can the drafter model operate in a smaller vocabulary space than the target model while maintaining  a similar acceptance rate?}. If so, this would cut-down the parameters in the bulky LM-head, significantly improving efficiency in memory-bound systems. 

\SA{First sentence needs to be reworded - it makes it seem like accuracy of draft is not important} Ultimately, the job of draft model is to aid the target model by predicting similar tokens without any emphasis on accuracy, as rejection sampling proves lossless generation \cite{OG spd paper}. \SA{Need to mention a point/data about how most of the tokens that end up being accepted are the same if this is the point we're trying to make -> } For the drafter model, therefore, even choosing a smaller subset of vocabulary would lead to similar accuracy while reducing the high computation and memory used due to LM-head. We show a simple way of finding appropriate subsets of vocabulary for drafter model based on the observed target model generations on downstream tasks. 

% In \cite{MLLM+SPD paper}, authors showed that the primary role of draft model was to predict easy words such as articles/prepositions and completing half-words owing the limited representation capacity of the draft model.

Another analogy of our efficient draft LM-head  is with the usage of LORA with LLMs \cite{}. Similar to LLMs finetuned on different LORA parameters for a particular downstream task to efficiently improve accuracy, in this work, we study the impact of different draft model vocabularies for improving the speed-up of SpD systems. We observe that for different tasks the frequency of tokens in the training set of that task is different and often following a long-tail of near zeros. In \cref{fig:xlam-bar-plot}, we show a special case of target model (Llama3.2-3B-Insturct) generations on the training split of function-calling dataset \cite{xlam}. Only a few tokens occur at high-frequency while majority of tokens in vocabulary don't occur at all. Specifically, $15$ tokens occur $> 10$k times, next $140$ tokens occur from $(1\text{k}, 10\text{k})$, while around $120,000$ tokens rarely occur. 
Motivated by this, in this work, we show that if we were to restrict the draft model to only predicting the most frequently occurring subset of the vocabulary, we may maintain accuracy while reducing the LM-Head size significantly \SA{by how much?}. We use Llama3 model family for our experiments and evaluate on Speculative benchmark, function-calling task \cite{}, and open-ended text generation \cite{dolly}.

\begin{figure}[]
    \centering
    \includegraphics[width=0.95\linewidth]{images/xlam-raw-dataset-answers.png}
    \caption{XLAM (function-calling) dataset token freqeuncy based on target model generation. Plots divided into three parts for ease of readability.}
    \label{fig:xlam-bar-plot}
\vspace{-0.5cm}
\end{figure}

The paper is divided into following sections: \color{red} complete this \color{black}


==> contents/03_method.tex <==

\section{Method}
\label{sec:method}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/draft-vocab-trimming-v1.png}
    \caption{Inference with trimmed vocabulary of draft model}
    \label{fig:main-diagram}
\vspace{-0.5cm}
\end{figure}

% \begin{itemize}
%     \item our method is simple and based on the observation that (1) small models are not able to predict all tokens, and (2) down-stream tasks might not use the entire vocabulary space of the model. \cref{fig:main-diagram}
%     \item we propose to cut-down the draft model vocabulary size using three approaches: (i) raw data based, (ii) target model generation based, (iii) draft model generation based. 
%     \item for each of these we count the frequency of tokens and keep the top-K tokens. The K decides the new vocabulary size, reducing the draft model size by hidden-dim $\times$ (V-K). 
% \end{itemize}

For any SpD technique, our method can be infused using simple steps: first, choose a calibration dataset (raw-text or target model generated), pick and store the Top-$K$ occurring tokens in this dataset (same as high probability tokens) \cref{eq:top-k}, second, compute a mapping between new draft vocabulary token index to original (or target) model token index, and third, a minor modification in the draft model generation implementation. The modifications in the draft model simply involve updating the LM-head to have a fewer number of rows instead of all the rows (\cref{eq:LM-head-draft}). Any token generated from draft model can then be passed through a mapping converting the drafter token index to target model token index. This final re-mapping step is necessary to enable target model verification. We use an array to map tokens from \ourmethod{} space to original space which consumes negligible time. A general flow of using trimmed draft model head during inference is shown in \cref{fig:main-diagram} with algorithm mentioned in \cref{algorithm:SpD_with_trimmed_vocab} in \cref{subsec:appendix_algo}.

\begin{align}
    t_{1},\dots, t_{K} = & \underset{j\in\{1,\dots,K\}}{\argmax}\,p_{\text{token},j} \label{eq:top-k}
    \\
    % LM_{\text{head},\text{draft}}' = & I_{t_{1}, \dots t_{K}}LM_{\text{head},\text{draft}} \label{eq:LM-head-draft}
    LM_{\text{head},\text{draft}}' = & LM_{\text{head},\text{draft}}[\Bar{t},:] \label{eq:LM-head-draft}
\end{align}
where, $p_{\text{token}}$ is the probability of token occurrence for given dataset $D$, and $\bar{t} =\{t_{1}, \dots t_{K}\}$. 
% is an indicator matrix to sub-select appropriate rows LM-head. 
% with each row a one-hot vector, and for any row $j$, only entry $i_{j}=1$. 
Our method helps save $d(V-K)$ memory and proportional compute, where $d$ is LLM hidden-state, $V$ is original vocabulary size, and $K$ is the reduced vocabulary size. For EAGLE \cite{li2024eagle}, the $LM_{\text{head},\text{draft}}=LM_{\text{head},\text{target}}$.

For the first step, we consider two types of datasets: (a) raw text data, and (b) target model generated data (also called distillation dataset). Raw text data is available in ample amounts, even for many evaluation tasks which have train splits. Distillation data is also often readily available as it is used to finetune the draft model. If not, it may be easily generated by simply allowing the target model to generate completions from a dataset. As an ablation, we additionally use draft model generated data (used for finetuning draft model in \cite{zhou2023distillspec}), finding, however, that the target model generated dataset performs the best as shown in \cref{tab:specbench_llama3b_table}. 

Given, or having constructed, such a dataset for a particular task, we then simply count the frequency of the tokens in the dataset and determine the Top-$K$ tokens. Here, $K$ is set to a choice much lower than the original vocabulary size, in our experiments we set $K=0.25V$ for spec-bench tasks while $K=0.04V$ for function-calling task. A lower $K$ will see some degradation in acceptance-rate but will reduce the overall draft model size, which will increase memory-bound speed-up. To find the optimal choice, we ablate over different $K$ in \cref{sec:results}.

Finally, with this Top-$K$ set available, we create a trimmed-down LM-head for the draft model, $ LM_{head, draft}' \in \mathbb{R}^{K \times d}$,  by picking rows corresponding to top-$K$ tokens from the target LM-head  $LM_{head, target}$. The draft model token index generations using the trimmed head are within $\{0,1,\dots, K\}$ which are then mapped back to target model vocabulary space ($\{t_{1}, t_{2}, \dots t_{K}\}$). 

Note that, in this paper, we restricted \ourmethod{} experiments to choose trimmed draft model LM-head based on Top-$K$, however, our framework is general and also supports choosing based on Top-$P$, or based on minimum frequency of tokens in caliberation datasets. 
Moreover, other selection criteria for trimmed vocabulary  can be: compute resources available, hardware-memory constraints, or maximum allowable drop in accuracy.
We leave it as future work to further experiments with these. 


==> tables/dolly_ablation_llama3b_eagle.tex <==
\begin{table}[]
    \caption{Eagle based SpD for Llama3.2-3B-Instruct model on open-ended text generation (DOLLY) with different sizes of draft-LM-head}
    \label{tab:eagle_llama3.2-3b-dolly-ablation}
    \begin{center}
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{l|c|c|c|c}
   Method  & tokens (K) & LM$_{\text{Head},\text{Draft}}$ (M) & BE & MBSU
    \\
    \bottomrule
   Baseline  & 128.3 & 394.0 & 3.237 & 1.520 
   \\
   \bottomrule
   \multirow{7}{*}{+Target generated} & 10240 & 31.4 & 2.951 & 1.758
   \\
                & 16.4  &  50.3 & 3.063 & 1.799
    \\
                &  22.5  & 69.2 & 3.140 & 1.820
    \\              
                &  33.0  & 101.3 & 3.193 & 1.809
    \\
                &  37.1  & 113.9 & 3.209 & 1.801
    \\
                &  45.3  & 139.0 & 3.227 & 1.780
    \\
                &  55.0  & 169.0 & 3.227 & 1.745
    \end{tabular}%
    }
\end{center}
\end{table}


==> tables/dolly_llama3b_independent_draft.tex <==
\begin{table}[]
    \caption{Independent-drafter based SpD for Llama3.2-3B model on open-ended text generation (DOLLY) and function calling (XLAM) task}
    \label{tab:indepdent_llama3.2-3b-dolly-xlam}
    \begin{center}
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{l|c|c|c|c|c|c}
   Method  & \multicolumn{3}{c}{DOLLY} & \multicolumn{3}{c}{XLAM} 
    \\
     \cmidrule[0.8pt](lr){2-4} \cmidrule[0.8pt](lr){5-7} 
    & LM$_{\text{Head},\text{Draft}}$ (M) & BE & MBSU & LM$_{\text{Head},\text{Draft}}$ (M) & BE & MBSU
    \\
    \cmidrule[0.8pt](lr){1-1} \cmidrule[0.8pt](lr){2-7}
   Baseline  & 131.3 &  3.675 & 2.642 & 131.3 & 2.364 & 1.700
   \\
   +Raw-dataset & 33.8 &  3.483 & 2.744 & 5.1 & 2.075 & 1.681
   \\
   +Target generated & 33.8  & 3.629 & 2.858 & 5.1 & 2.344 & 1.900
   \\
   +Draft generated & 33.8 & 3.589 & 2.827 & 5.1 & 2.314 & 1.875
   \\
    \end{tabular}
    }
\end{center}
\end{table}

